Competitive Facility Location with Market Expansion and Customer-centric Objective

We study a competitive facility location problem, where customer behavior is modeled and predicted using a discrete choice random utility model. The goal is to strategically place new facilities to maximize the overall captured customer demand in a competitive marketplace. In this work, we introduce two novel considerations. First, the total customer demand in the market is not fixed but is modeled as an increasing function of the customers' total utilities. Second, we incorporate a new term into the objective function, aiming to balance the firm's benefits and customer satisfaction. Our new formulation exhibits a highly nonlinear structure and is not directly solved by existing approaches. To address this, we first demonstrate that, under a concave market expansion function, the objective function is concave and submodular, allowing for a $(1-1/e)$ approximation solution by a simple polynomial-time greedy algorithm. We then develop a new method, called Inner-approximation, which enables us to approximate the mixed-integer nonlinear problem (MINLP), with arbitrary precision, by an MILP without introducing additional integer variables. We further demonstrate that our inner-approximation method consistently yields lower approximations than the outer-approximation methods typically used in the literature. Moreover, we extend our settings by considering a\textit{ general (non-concave)} market-expansion function and show that the Inner-approximation mechanism enables us to approximate the resulting MINLP, with arbitrary precision, by an MILP. To further enhance this MILP, we show how to significantly reduce the number of additional binary variables by leveraging concave areas of the objective function. Extensive experiments demonstrate the efficiency of our approaches.

==> tables/concave_cap.tex <==
\begin{table}
\centering
\caption{Results on the ORlib dataset.}
\label{table:orlib_cc}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\hline
\multirow{2}{*}{Dataset} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cline{3-5} \cline{7-9} \cline{11-13} 
                            &  & PIA                           & OA                            & LS                            &  & PIA                               & OA                              & LS                              &  & PIA                          & OA                                  & LS                          \\ \hline
cap101                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.282                  & 0.112                          & \textbf{0.054}                 \\
cap102                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.240                  & 0.131                          & \textbf{0.055}                 \\
cap103                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.246                  & 0.083                          & \textbf{0.055}                 \\
cap104                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.268                  & 0.124                          & \textbf{0.055}                 \\
cap131                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.740                  & \textbf{0.126}                 & 0.317                          \\
cap132                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.794                  & \textbf{0.168}                 & 0.316                          \\
cap133                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.725                  & \textbf{0.179}                 & 0.317                          \\
cap134                   &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 0.767                  & \textbf{0.147}                 & 0.316                          \\
capa                     &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 13.382                 & \textbf{7.394}                 & 55.520                         \\
capb                     &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 12.901                 & \textbf{7.215}                 & 53.387                         \\
capc                     &  & \textbf{81}                & \textbf{81}               & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & 13.768                 & \textbf{7.584}                 & 53.889                         \\ \midrule
Total                    &  & \textbf{891}               & \textbf{891}              & \textbf{891}              &  & \textbf{891}                 & \textbf{891}                 & \textbf{891}                 &  & -                      & -                              & -                              \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/concave_hm14.tex <==
\begin{table}
\centering
\caption{Results on the HM14 dataset.}
\label{table:hm14_cc}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}rrlccclccclccc@{}}
\toprule
\multirow{2}{*}{$N$} & \multirow{2}{*}{$m$} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No. of \\ solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No. of \\ inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average\\ computing time (s)\end{tabular}} \\ \cmidrule(lr){4-6} \cmidrule(lr){8-10} \cmidrule(l){12-14} 
                     &                      &  & PIA                         & OA                          & LS                         &  & PIA                            & OA                            & LS                            &  & PIA                             & OA                    & LS                             \\ \midrule
50                   & 25                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & 0.167                           & 0.087                 & \textbf{0.054}                 \\
50                   & 50                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.034}                  & 0.129                 & 0.316                          \\
50                   & 100                  &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.036}                  & 0.057                 & 2.514                          \\
100                  & 25                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.045}                  & 0.231                 & 0.084                          \\
100                  & 50                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.043}                  & 0.074                 & 0.605                          \\
100                  & 100                  &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.072}                  & 0.123                 & 4.991                          \\
200                  & 25                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.050}                  & 0.060                 & 0.144                          \\
200                  & 50                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.090}                  & 0.128                 & 1.176                          \\
200                  & 100                  &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.166}                  & 0.351                 & 10.004                         \\
400                  & 25                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.118}                  & 0.199                 & 0.260                          \\
400                  & 50                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.216}                  & 0.373                 & 2.328                          \\
400                  & 100                  &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.495}                  & 1.305                 & 20.620                         \\
800                  & 25                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.287}                  & 0.588                 & 0.498                          \\
800                  & 50                   &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{0.908}                  & 1.331                 & 4.604                          \\
800                  & 100                  &  & \textbf{81}                 & \textbf{81}                 & \textbf{81}                &  & \textbf{81}                    & \textbf{81}                   & \textbf{81}                   &  & \textbf{1.542}                  & 3.043                 & 41.417                         \\ \midrule
\multicolumn{2}{l}{Total}                   &  & \textbf{1215}               & \textbf{1215}               & \textbf{1215}              &  & \textbf{1215}                  & \textbf{1215}                 & \textbf{1215}                 &  & -                               & -                     & -                              \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/concave_nyc.tex <==
\begin{table}
\centering
\caption{Results on the NYC dataset.}
\label{table:nyc_cc}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multirow{2}{*}{$C$} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No. of \\ solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No. of \\ inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average\\ computing time (s)\end{tabular}} \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} \cmidrule(l){11-13} 
                     &  & PIA                        & OA                        & LS                        &  & PIA                          & OA                           & LS                           &  & PIA                           & OA                       & LS                            \\ \midrule
2                    &  & \textbf{9}                 & \textbf{9}                & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1090.6                        & 5098.4                   & \textbf{67.4}                 \\
3                    &  & \textbf{9}                 & 8                         & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1360.0                        & 3641.2                   & \textbf{185.9}                \\
4                    &  & \textbf{9}                 & 8                         & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1322.9                        & 3734.6                   & \textbf{355.3}                \\
5                    &  & \textbf{9}                 & 8                         & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1567.1                        & 6080.4                   & \textbf{576.5}                \\
6                    &  & \textbf{9}                 & 7                         & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1592.2                        & 2855.4                  & \textbf{838.8}                \\
7                    &  & \textbf{9}                 & \textbf{9}                & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1436.7                        & 4317.1                   & \textbf{1081.3}               \\
8                    &  & \textbf{9}                 & \textbf{9}                & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & 1627.2                        & 3637.2                   & \textbf{1570.4}               \\
9                    &  & \textbf{9}                 & \textbf{9}                & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & \textbf{1502.2}               & 4937.4                   & 1668.6                        \\
10                   &  & \textbf{9}                 & \textbf{9}                & \textbf{9}                &  & \textbf{9}                   & \textbf{9}                   & \textbf{9}                   &  & \textbf{1405.4}               & 6524.3                   & 2420.6                        \\ \midrule
Total                &  & \textbf{81}                & 76                        & \textbf{81}               &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                  &  & -                             & \textbf{-}               & -                             \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/concave_union.tex <==
\begin{table}
\centering
\caption{Results on the HM14 dataset.}
\label{table:concave_union}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}clllllccclccclccc@{}}
\toprule
\multirow{2}{*}{Dataset} &  & \multirow{2}{*}{$N$} &  & \multirow{2}{*}{$m$} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cmidrule(lr){7-9} \cmidrule(lr){11-13} \cmidrule(l){15-17} 
                         &  &                      &  &                      &  & PIA                          & OA                          & LS                           &  & PIA                             & OA                             & LS                             &  & PIA                            & OA                            & LS                              \\ \midrule
HM14                     &  & 50                   &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & 0.17                           & 0.09                          & \textbf{0.05}                   \\
HM14                     &  & 50                   &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.03}                  & 0.13                          & 0.32                            \\
HM14                     &  & 50                   &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.04}                  & 0.06                          & 2.51                            \\
HM14                     &  & 100                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.04}                  & 0.23                          & 0.08                            \\
HM14                     &  & 100                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.04}                  & 0.07                          & 0.60                            \\
HM14                     &  & 100                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.07}                  & 0.12                          & 4.99                            \\
HM14                     &  & 200                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.05}                  & 0.06                          & 0.14                            \\
HM14                     &  & 200                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.09}                  & 0.13                          & 1.18                            \\
HM14                     &  & 200                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.17}                  & 0.35                          & 10.00                           \\
HM14                     &  & 400                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.12}                  & 0.20                          & 0.26                            \\
HM14                     &  & 400                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.22}                  & 0.37                          & 2.33                            \\
HM14                     &  & 400                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.49}                  & 1.31                          & 20.62                           \\
HM14                     &  & 800                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.29}                  & 0.59                          & 0.50                            \\
HM14                     &  & 800                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.91}                  & 1.33                          & 4.60                            \\
HM14                     &  & 800                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{1.54}                  & 3.04                          & 41.42                           \\ \midrule
cap\_10                  &  & 50                   &  & 25                   &  & \textbf{324}                 & \textbf{324}                & \textbf{324}                 &  & \textbf{324}                    & \textbf{324}                   & \textbf{324}                   &  & 0.26                           & 0.11                          & \textbf{0.05}                   \\
cap\_13                  &  & 50                   &  & 50                   &  & \textbf{324}                 & \textbf{324}                & \textbf{324}                 &  & \textbf{324}                    & \textbf{324}                   & \textbf{324}                   &  & 0.76                           & \textbf{0.16}                 & 0.32                            \\
cap\_abc                 &  & 1000                 &  & 100                  &  & \textbf{243}                 & \textbf{243}                & \textbf{243}                 &  & \textbf{243}                    & \textbf{243}                   & \textbf{243}                   &  & 13.35                          & \textbf{7.40}                 & 54.27                           \\ \midrule
NYC                      &  & 82341                &  & 59                   &  & \textbf{81}                  & 76                          & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & 1433.80                        & 5547.00                       & \textbf{973.86}                 \\ \midrule
\multicolumn{5}{c}{Total}                                                    &  & \textbf{2187}                & 2182                        & \textbf{2187}                &  & \textbf{2187}                   & \textbf{2187}                  & \textbf{2187}                  &  & -                              & -                             & -                               \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/epsilon_error.tex <==
\begin{table}
\centering
\caption{Results of PIA method on different settings of parameter $\epsilon$.}
\label{table:hm14_cc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccclcclcclcclcclcc@{}}
\toprule
\multirow{2}{*}{m} & \multicolumn{2}{c}{$\epsilon= 1E-5$} &  & \multicolumn{2}{c}{$\epsilon =1E-4$} &  & \multicolumn{2}{c}{$\epsilon = 1E-3$} &  & \multicolumn{2}{c}{$\epsilon = 1E-2$} &  & \multicolumn{2}{c}{$\epsilon =1E-1$} &  & \multicolumn{2}{c}{$\epsilon =1E+0$} \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9} \cmidrule(lr){11-12} \cmidrule(lr){14-15} \cmidrule(l){17-18} 
                   & Error (\%)      & Runtime (s)     &  & Error (\%)      & Runtime (s)     &  & Error (\%)      & Runtime (s)     &  & Error (\%)      & Runtime (s)     &  & Error (\%)      & Runtime (s)     &  & Error (\%)      & Runtime (s)     \\ \midrule
25                 & 0          & 4.82        &  & 0          & 1.74        &  & 0          & 0.937       &  & 0          & 0.709       &  & 0          & 0.641       &  & 0          & 0.627       \\
50                 & 0          & 6.685       &  & 0          & 2.401       &  & 0          & 1.244       &  & 0          & 0.928       &  & 0          & 0.782       &  & 0.031      & 0.734       \\
100                & 0          & 5.597       &  & 0          & 2.194       &  & 0          & 1.185       &  & 0          & 1.009       &  & 0.066      & 0.877       &  & 0.066      & 0.915       \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/market_expansion.tex <==
\begin{table}
\centering
\caption{Impacts of the slope of the market expansion function.}
\label{table:market_expansion}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}rlrlccclccclccc@{}}
\toprule
\multirow{2}{*}{$\alpha$} &  & \multirow{2}{*}{Dataset} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cmidrule(lr){5-7} \cmidrule(lr){9-11} \cmidrule(l){13-15} 
                          &  &                          &  & PIA                          & OA                           & LS                          &  & PIA                             & OA                             & LS                             &  & PIA                         & OA                                   & LS                          \\ \midrule
1                         &  & cap10                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & \textbf{324}                   & \textbf{324}                   &  & 0.022                       & \textbf{0.015}                       & 0.061                       \\
1                         &  & cap13                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & \textbf{324}                   & \textbf{324}                   &  & 0.028                       & \textbf{0.022}                       & 0.328                       \\
5                         &  & cap10                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 268                            & 308                            &  & 0.817                       & \textbf{0.006}                       & 0.059                       \\
5                         &  & cap13                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 288                            & 276                            &  & 0.493                       & \textbf{0.009}                       & 0.327                       \\
10                        &  & cap10                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 260                            & \textbf{324}                   &  & 0.514                       & \textbf{0.008}                       & 0.059                       \\
10                        &  & cap13                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 296                            & 312                            &  & 0.402                       & \textbf{0.012}                       & 0.327                       \\
20                        &  & cap10                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 260                            & 316                            &  & 0.293                       & \textbf{0.009}                       & 0.059                       \\
20                        &  & cap13                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 296                            & \textbf{324}                   &  & 0.235                       & \textbf{0.013}                       & 0.327                       \\
50                        &  & cap10                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 288                            & \textbf{324}                   &  & 0.151                       & \textbf{0.010}                       & 0.059                       \\
50                        &  & cap13                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 312                            & \textbf{324}                   &  & 0.138                       & \textbf{0.014}                       & 0.327                       \\
100                       &  & cap10                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 288                            & \textbf{324}                   &  & 0.092                       & \textbf{0.011}                       & 0.059                       \\
100                       &  & cap13                    &  & \textbf{324}                 & \textbf{324}                 & \textbf{324}                &  & \textbf{324}                    & 316                            & \textbf{324}                   &  & 0.093                       & \textbf{0.015}                       & 0.327                       \\ \midrule
\multicolumn{3}{c}{Total}                               &  & \textbf{3888}                & \textbf{3888}                & \textbf{3888}               &  & \textbf{3888}                   & 3520                           & 3804                           &  & -                           & -                                    & -                           \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/nonconcave_cap.tex <==
\begin{table}
\centering
\caption{Results on the ORLIB dataset.}
\label{table:orlib_noncc}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\hline
\multirow{2}{*}{Dataset} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cline{3-5} \cline{7-9} \cline{11-13} 
                            &  & PIA                           & OA                            & LS                            &  & PIA                               & OA                              & LS                              &  & PIA                          & OA                                  & LS                          \\ \hline
cap101                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 67                              & 77                              &  & 0.460                        & \textbf{0.006}                      & 0.059                       \\
cap102                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 67                              & 77                              &  & 0.472                        & \textbf{0.006}                      & 0.059                       \\
cap103                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 67                              & 77                              &  & 0.685                        & \textbf{0.006}                      & 0.060                       \\
cap104                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 67                              & 77                              &  & 0.678                        & \textbf{0.006}                      & 0.060                       \\
cap131                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 72                              & 69                              &  & 0.663                        & \textbf{0.009}                      & 0.324                       \\
cap132                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 72                              & 69                              &  & 0.624                        & \textbf{0.009}                      & 0.324                       \\
cap133                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 72                              & 69                              &  & 0.652                        & \textbf{0.009}                      & 0.322                       \\
cap134                      &  & \textbf{81}                   & \textbf{81}                   & \textbf{81}                   &  & \textbf{81}                       & 72                              & 69                              &  & 0.642                        & \textbf{0.009}                      & 0.326                       \\
capa                        &  & 73                            & \textbf{81}                   & \textbf{81}                   &  & 80                                & 80                              & \textbf{81}                     &  & 57.959                       & \textbf{1.544}                      & 57.411                      \\
capb                        &  & 76                            & \textbf{81}                   & \textbf{81}                   &  & \textbf{80}                       & \textbf{80}                     & \textbf{80}                     &  & 29.768                       & \textbf{1.607}                      & 56.756                      \\
capc                        &  & 73                            & \textbf{81}                   & \textbf{81}                   &  & 80                                & \textbf{81}                     & \textbf{81}                     &  & 21.577                       & \textbf{1.525}                      & 57.334                      \\ \hline
Total                       &  & 870                           & \textbf{891}                  & \textbf{891}                  &  & \textbf{888}                      & 797                             & 826                             &  & -                            & -                                   & -                           \\ \hline
\end{tabular}}
\end{table}

==> tables/nonconcave_hm14.tex <==
\begin{table}
\centering
\caption{Results on the HM14 dataset.}
\label{table:hm14_noncc}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}rrcccccccccccc@{}}
\toprule
\multirow{2}{*}{$N$} & \multirow{2}{*}{$m$} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cmidrule(lr){4-6} \cmidrule(lr){8-10} \cmidrule(l){12-14} 
                     &                      &  & PIA                          & OA                           & LS                          &  & PIA                             & OA                             & LS                             &  & PIA                                  & OA                          & LS                          \\ \midrule
50                   & 25                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.035}                       & 0.211                       & 0.061                       \\
50                   & 50                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.027}                       & 0.084                       & 0.320                       \\
50                   & 100                  &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.081}                       & 0.046                       & 2.534                       \\
100                  & 25                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.025}                       & 0.205                       & 0.087                       \\
100                  & 50                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.068}                       & 0.067                       & 0.611                       \\
100                  & 100                  &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.044}                       & 0.107                       & 5.040                       \\
200                  & 25                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.059}                       & 0.056                       & 0.146                       \\
200                  & 50                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.059}                       & 0.108                       & 1.204                       \\
200                  & 100                  &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.089}                       & 0.284                       & 10.067                      \\
400                  & 25                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.084}                       & 0.189                       & 0.265                       \\
400                  & 50                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.117}                       & 0.339                       & 2.361                       \\
400                  & 100                  &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.187}                       & 0.972                       & 20.501                      \\
800                  & 25                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.182}                       & 0.580                       & 0.502                       \\
800                  & 50                   &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.276}                       & 1.283                       & 4.722                       \\
800                  & 100                  &  & \textbf{81}                  & \textbf{81}                  & \textbf{81}                 &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & \textbf{0.462}                       & 2.683                       & 43.184                      \\ \midrule
\multicolumn{2}{c}{Total}                   &  & \textbf{1215}                & \textbf{1215}                & \textbf{1215}               &  & \textbf{1215}                   & \textbf{1215}                  & \textbf{1215}                  &  & -                                    & -                           & -                           \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/nonconcave_nyc.tex <==
\begin{table}
\centering
\caption{Results on the NYC dataset.}
\label{table:nyc_noncc}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multirow{2}{*}{$C$} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cmidrule(lr){3-5} \cmidrule(lr){7-9} \cmidrule(l){11-13} 
                     &  & PIA                          & OA                          & LS                           &  & PIA                             & OA                             & LS                             &  & PIA                                & OA                       & LS                               \\ \midrule
2                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & 634.1                              & 3746.7                   & \textbf{71.8}                    \\
3                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & 640.9                              & 4250.6                   & \textbf{188.7}                   \\
4                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & 632.6                              & 2862.7                   & \textbf{354.8}                   \\
5                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & 673.7                              & 4273.5                   & \textbf{568.7}                   \\
6                    &  & \textbf{9}                   & 8                           & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & \textbf{627.6}                     & 3626.3                   & 805.9                            \\
7                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & \textbf{670.7}                     & 4385.8                   & 1217.1                           \\
8                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & \textbf{673.3}                     & 4361.5                   & 1456.7                           \\
9                    &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & \textbf{1100.3}                    & 4122.2                   & 1931.0                           \\
10                   &  & \textbf{9}                   & \textbf{9}                  & \textbf{9}                   &  & \textbf{9}                      & \textbf{9}                     & \textbf{9}                     &  & \textbf{787.3}                     & 4862.8                   & 2074.5                           \\ \midrule
Total                &  & \textbf{81}                  & 80                          & \textbf{81}                  &  & \textbf{81}                     & \textbf{81}                    & \textbf{81}                    &  & -                                  & -                        & -                                \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/nonconcave_union.tex <==
\begin{table}
\centering
\caption{Comparison results for non-concave market expansion.}
\label{table:nonconcave_union}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}clllllccclccclccc@{}}
\toprule
\multirow{2}{*}{Dataset} &  & \multirow{2}{*}{$N$} &  & \multirow{2}{*}{$m$} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      solved inst.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}No.   of \\      inst. with best obj.\end{tabular}} &  & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}Average   \\      computing time (s)\end{tabular}} \\ \cmidrule(lr){7-9} \cmidrule(lr){11-13} \cmidrule(l){15-17} 
                         &  &                      &  &                      &  & PIA                          & OA                          & LS                           &  & PIA                              & OA                            & LS                             &  & PIA                                & OA                               & LS                       \\ \midrule
HM14                     &  & 50                   &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.04}                      & 0.21                             & 0.06                     \\
HM14                     &  & 50                   &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.03}                      & 0.08                             & 0.32                     \\
HM14                     &  & 50                   &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & 0.08                               & \textbf{0.05}                    & 2.53                     \\
HM14                     &  & 100                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.03}                      & 0.20                             & 0.09                     \\
HM14                     &  & 100                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.07}                      & \textbf{0.07}                    & 0.61                     \\
HM14                     &  & 100                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.04}                      & 0.11                             & 5.04                     \\
HM14                     &  & 200                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.06}                      & \textbf{0.06}                    & 0.15                     \\
HM14                     &  & 200                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.06}                      & 0.11                             & 1.20                     \\
HM14                     &  & 200                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.09}                      & 0.28                             & 10.07                    \\
HM14                     &  & 400                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.08}                      & 0.19                             & 0.26                     \\
HM14                     &  & 400                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.12}                      & 0.34                             & 2.36                     \\
HM14                     &  & 400                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.19}                      & 0.97                             & 20.50                    \\
HM14                     &  & 800                  &  & 25                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.18}                      & 0.58                             & 0.50                     \\
HM14                     &  & 800                  &  & 50                   &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.28}                      & 1.28                             & 4.72                     \\
HM14                     &  & 800                  &  & 100                  &  & \textbf{81}                  & \textbf{81}                 & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{0.46}                      & 2.68                             & 43.18                    \\ \midrule
cap\_10                  &  & 50                   &  & 25                   &  & \textbf{324}                 & \textbf{324}                & \textbf{324}                 &  & \textbf{324}                     & 268                           & 308                            &  & 0.57                               & \textbf{0.01}                    & 0.06                     \\
cap\_13                  &  & 50                   &  & 50                   &  & \textbf{324}                 & \textbf{324}                & \textbf{324}                 &  & \textbf{324}                     & 288                           & 276                            &  & 0.65                               & \textbf{0.01}                    & 0.32                     \\
cap\_abc                 &  & 1000                 &  & 100                  &  & 222                          & \textbf{243}                & \textbf{243}                 &  & 240                              & 241                           & \textbf{242}                   &  & 36.43                              & \textbf{1.56}                    & 57.17                    \\ \midrule
NYC                      &  & 82341                &  & 59                   &  & \textbf{81}                  & 80                          & \textbf{81}                  &  & \textbf{81}                      & \textbf{81}                   & \textbf{81}                    &  & \textbf{715.62}                    & 4258.47                          & 963.25                   \\ \midrule
\multicolumn{5}{c}{Total}                                                    &  & 2166                         & 2186                        & \textbf{2187}                &  & \textbf{2184}                    & 2093                          & 2122                           &  & -                                  & -                                & -                        \\ \bottomrule
\end{tabular}}
\end{table}
